FedGKD: Unleashing the Power of Collaboration in Federated Graph Neural Networks

Federated training of Graph Neural Networks (GNN) has become popular in recent years due to its ability to perform graph-related tasks under data isolation scenarios while preserving data privacy. However, graph heterogeneity issues in federated GNN systems continue to pose challenges. Existing frameworks address the problem by representing local tasks using different statistics and relating them through a simple aggregation mechanism. However, these approaches suffer from limited efficiency from two aspects: low quality of task-relatedness quantification and inefficacy of exploiting the collaboration structure. To address these issues, we propose FedGKD, a novel federated GNN framework that utilizes a novel client-side graph dataset distillation method to extract task features that better describe task-relatedness, and introduces a novel server-side aggregation mechanism that is aware of the global collaboration structure. We conduct extensive experiments on six real-world datasets of different scales, demonstrating our framework's outperformance.

==> gumbel_softmax_issue.tex <==
\section{Current issue on gumbel softmax/sigmoid}
The description of the procedure in the main text appears problematic. Recall that for nodes $u, v$, our initial attempt is to formulate the probabilistic model of the distilled graph as:
\begin{align}
    \mathbb{P}[A_{uv} = 1] = \dfrac{e^{\langle x_u, x_v\rangle}}{1 + e^{\langle x_u, x_v\rangle}} = \dfrac{e^{\langle x_u, x_v\rangle}}{e^0 + e^{\langle x_u, x_v\rangle}}
\end{align}
According to standard gumbel-softmax trick, with two categories the relaxation is written as
\begin{align}
    q_{uv} = \dfrac{e^{\left(\langle x_u, x_v\rangle + \omega\right) / \tau}}{e^{\omega^\prime/\tau} + e^{\left(\langle x_u, x_v\rangle + \omega\right) / \tau}} = \dfrac{e^{\left(\langle x_u, x_v\rangle + \omega - \omega^\prime\right) / \tau}}{1 + e^{\left(\langle x_u, x_v\rangle + \omega - \omega^\prime\right) / \tau}},
\end{align}
where $\omega$ and $\omega^\prime$ are independently sampled from standard gumbel distribution. The validity of gumbel-softmax relaxation says essentially the following:
\begin{align}
    \lim_{\tau \rightarrow 0} \mathbb{P}[q_{uv} = 1] = \mathbb{P}[A_{uv} = 1]
\end{align}
From the code implementation, it is worth noting that if we instead want to apply sigmoid function to perturbed logits directly, the perturbation shall be the difference of two independent gumbels (actually this yields a logistic distribution), which is also used in some NLP applications \cite{geng2020does} and the PGExplainer for GNN interpretation \cite{luo2020parameterized}. The current implementation used gumbel directly, which is problematic.
\paragraph{Controlling for sparsity} yet another issue is the attempt to control sparsity level which affects the overall performance of the proposed framework. From the code implementation, I found that the forward computation is sparsified, i.e.
\begin{align}
    \widehat{A}_{uv} = \mathbf{1}_{q_{uv} > \rho},
\end{align}
while the backward pass is based on $q_{uv}$s directly. I guess this is inspired by the straight-through trick \cite{jang2016categorical} which was also implemented in \texttt{torch.nn.functional.gumbel\_softmax} api via setting \texttt{hard $=$ True}. However, a sparsified forward pass with a non-sparsified backward pass is problematic. Careful reviewers (assume we are sufficiently unlucky to encounter one) may mess around with this, especially if $\rho$ is involved in the ablation. 
\paragraph{Suggested fix} We return to the definition of $q_{uv}$, the expected sparsity level is by definition:
\begin{align}
    \frac{1}{\left|V\right|^2}\sum_{u \in V, v \in V} \mathbb{P}[A_{uv} = 1] = \frac{1}{\left|V\right|^2}\mathbb{E}\left[\lim_{\tau \rightarrow 0}\sum_{u \in V, v \in V} q_{uv}\right].
\end{align}
Now via monotonicity of $q_{uv}$s, a straightforward solution is to add a penalty:
\begin{align}\label{eq:sparsity_penalty}
    q_{uv}(\gamma)= \dfrac{e^{\left(\langle x_u, x_v\rangle - {\color{red}\gamma} + \omega - \omega^\prime\right) / \tau}}{1 + e^{\left(\langle x_u, x_v\rangle - {\color{red}\gamma} + \omega - \omega^\prime\right) / \tau}},
\end{align}
with $\gamma > 0$. Now we bound the sparsity of the limiting case of \eqref{eq:sparsity_penalty}. For notational simplicity we set $\alpha = e^{-\gamma}$ and $\beta = \langle x_u, x_v \rangle$. Let when $\tau$ limits to zero, the ratio between the sparsified and the non-sparsified version is
\begin{align}\label{eq:sparsity_ratio}
    \dfrac{\frac{\alpha e^\beta}{1 + \alpha e^\beta}}{\frac{e^\beta}{1 + e^\beta}} = \alpha \left(1 + \dfrac{1 - \alpha}{e^{-\beta} + \alpha}\right)
\end{align}
from \eqref{eq:sparsity_ratio} we find that so long as $\left|\langle x_u, x_v \rangle\right|$ is bounded, we may get a formal certificate of sparsity. For example if all the $x_u$s are of unit length, then the sparsity ratio with penalty $\gamma$ is bounded from above by
\begin{align}
    e^{-\gamma} \left(1 + \dfrac{1 - e^{-\gamma}}{e^{-1} + e^{-\gamma}}\right)
\end{align}
The above ratio seems to be pretty OK, for example if we set $\gamma = 1$, we get a sparsity ratio of $0.68$. Note that this number holds uniformly across all nodes, which is potentially much greater than the actual sparsity level. 
